Granular convergence as an iterated local map

Granular convergence is a property of a granular pack as it is repeatedly sheared in a cyclic, quasistatic fashion, as the packing configuration changes via discrete events. Under suitable conditions the set of microscopic configurations encountered converges to a periodic sequence after sufficient shear cycles. Prior work modeled this evolution as the iteration of a pre-determined, random map from a set of discrete configurations into itself. Iterating such a map from a random starting point leads to similar periodic repetition. This work explores the effect of restricting the randomness of such maps in order to account for the local nature of the discrete events. The number of cycles needed for convergence shows similar statistical behavior to that of numerical granular experiments. The number of cycles in a repeating period behaves only qualitatively like these granular studies.

==> backmatter.tex <==
\begin{figure}
    \includegraphics[width=0.4\textwidth]{figures/experiment/expcycleconvergence.png}
    \caption{Graphs for strain amplitudes of distance $R(n)$ versus cycle number $n$ after \cite{Regev:2015fk}.   $\gamma = 0.06, 0.07, 0.075, 0.085, 0.088, 0.09, 0.093, 0.095$ from left to right. Inset shows graphs from strain amplitudes $\gamma = 0.12$ (blue) and $\gamma = 0.15$ (green), for which there was never a limiting cycle achieved.  See also Ref. \cite{Lavrentovich:2017rz} for similar findings.}
    %\label{fig:enter-label}
\end{figure}

\begin{figure}
    \includegraphics[width=0.4\textwidth]{figures/experiment/gamma = 0.088.png}
    \caption{$R(n)$ for $\gamma = 0.088$ with exponential fit. Ref: Regev et al}
    %\label{fig:enter-label}
\end{figure}

\begin{figure}
    \includegraphics[width=0.4\textwidth]{figures/experiment/gamma = 0.09.png}
    \caption{$R(n)$ for $\gamma = 0.09$ with exponential fit. Ref: Regev et al}
    %\label{fig:enter-label}
\end{figure}


\begin{figure}
    \includegraphics[width=0.4\textwidth]{figures/experiment/gamma = 0.095.png}
    \caption{$R(n)$ for $\gamma = 0.095$ with exponential fit. Ref: Regev et al}
    %\label{fig:enter-label}
\end{figure}


\begin{figure}
    \includegraphics[width=0.4\textwidth]{figures/experiment/tail_distributionwithexpfit.png}
    \caption{Tail length frequency count for 5000 generated graphs. The graph is well fitted with an exponential decay function.}
    %\label{fig:enter-label}
\end{figure}


\section*{Conclusion}

\backmatter

\bmhead{Supplementary information}

If your article has accompanying supplementary file/s please state so here. 

Authors reporting data from electrophoretic gels and blots should supply the full unprocessed scans for key as part of their Supplementary information. This may be requested by the editorial team/s if it is missing.

Please refer to Journal-level guidance for any specific requirements.

\bmhead{Acknowledgments}

Acknowledgments are not compulsory. Where included they should be brief. Grant or contribution numbers may be acknowledged.

Please refer to Journal-level guidance for any specific requirements.

\section*{Declarations}

Some journals require declarations to be submitted in a standardised format. Please check the Instructions for Authors of the journal to which you are submitting to see if you need to complete this section. If yes, your manuscript must contain the following sections under the heading `Declarations':

\begin{itemize}
\item Funding
\item Conflict of interest/Competing interests (check journal-specific guidelines for which heading to use)
\item Ethics approval 
\item Consent to participate
\item Consent for publication
\item Availability of data and materials
\item Code availability 
\item Authors' contributions
\end{itemize}


\appendix

\section{Appendixes}

\bibliography{MovshevaWitten2023}% Produces the bibliography via BibTeX.



\end{document}




\begin{figure}[h]%
\centering
\includegraphics[width=0.9\textwidth]{fig.eps}
\caption{This is a widefig. This is an example of long caption this is an example of long caption  this is an example of long caption this is an example of long caption}\label{fig1}
\end{figure}




==> unused_figure_captions.tex <==


\begin{figure}
    \includegraphics[width=0.4\textwidth]{figures/experiment/gamma = 0.088.png}
    \caption{$R(n)$ for $\gamma = 0.088$ with exponential fit. Ref: Regev et al}
    %\label{fig:enter-label}
\end{figure}

\begin{figure}
    \includegraphics[width=0.4\textwidth]{figures/experiment/gamma = 0.09.png}
    \caption{$R(n)$ for $\gamma = 0.09$ with exponential fit. Ref: Regev et al}
    %\label{fig:enter-label}
\end{figure}


\begin{figure}
    \includegraphics[width=0.4\textwidth]{figures/experiment/gamma = 0.095.png}
    \caption{$R(n)$ for $\gamma = 0.095$ with exponential fit. Ref: Regev et al}
    %\label{fig:enter-label}
\end{figure}

